Memory-Consistent Neural Networks for Imitation Learning

Imitation learning considerably simplifies policy synthesis compared to alternative approaches by exploiting access to expert demonstrations. For such imitation policies, errors away from the training samples are particularly critical. Even rare slip-ups in the policy action outputs can compound quickly over time, since they lead to unfamiliar future states where the policy is still more likely to err, eventually causing task failures. We revisit simple supervised ``behavior cloning'' for conveniently training the policy from nothing more than pre-recorded demonstrations, but carefully design the model class to counter the compounding error phenomenon. Our ``memory-consistent neural network'' (MCNN) outputs are hard-constrained to stay within clearly specified permissible regions anchored to prototypical ``memory'' training samples. We provide a guaranteed upper bound for the sub-optimality gap induced by MCNN policies. Using MCNNs on 10 imitation learning tasks, with MLP, Transformer, and Diffusion backbones, spanning dexterous robotic manipulation and driving, proprioceptive inputs and visual inputs, and varying sizes and types of demonstration data, we find large and consistent gains in performance, validating that MCNNs are better-suited than vanilla deep neural networks for imitation learning applications. Website: https://sites.google.com/view/mcnn-imitation

==> algorithm_3.tex <==

\begin{algorithm}
\caption{Behavior Cloning with Memory-Consistent Neural Networks: Evaluation}
\label{alg:mcnn_bc}
\hspace*{\algorithmicindent} \textbf{Input:} learned policy $f_{\theta}$, memory buffer $\mathcal{D}_M$, env, total evaluation trajectories $E$. \\
\hspace*{\algorithmicindent} \textbf{Output:} Normalized score
\begin{algorithmic}[1] % The number tells where the line numbering should start
\FOR{ep$=1$ to $E$}
    \STATE $s_t$ = env.reset()
    \STATE done = False
    \WHILE{not done}
        \STATE Find memory $(m_t^s, m_t^a) = \argmin_{\mathcal{D}_M} ||s_t-m_t^s||_2$ in memory buffer.
        \STATE Predict action as $a_t = f_{\theta}(s_t, m_t^s, m_t^a)$.
        \STATE $s_{t+1}, r_t, d_t, \_$ = env.step($a_t$)
        \STATE $s_{t}=s_{t+1}$
        \STATE Sum up rewards into $R_{\text{ep}}$
    \ENDWHILE
\ENDFOR 
\STATE Compute mean of episode rewards and corresponding D4RL normalized score \citep{fu2020d4rl}.
% \RETURN 
\end{algorithmic}
\end{algorithm}
